How to Query An Oracle? Efficient Strategies to Label Data

We consider the basic problem of querying an expert oracle for labeling a dataset in machine learning. This is typically an expensive and time consuming process and therefore, we seek ways to do so efficiently. The conventional approach involves comparing each sample with (the representative of) each class to find a match. In a setting with $N$ equally likely classes, this involves $N/2$ pairwise comparisons (queries per sample) on average. We consider a $k$-ary query scheme with $k\ge 2$ samples in a query that identifies (dis)similar items in the set while effectively exploiting the associated transitive relations. We present a randomized batch algorithm that operates on a round-by-round basis to label the samples and achieves a query rate of $O(\frac{N}{k^2})$. In addition, we present an adaptive greedy query scheme, which achieves an average rate of $\approx 0.2N$ queries per sample with triplet queries. For the proposed algorithms, we investigate the query rate performance analytically and with simulations. Empirical studies suggest that each triplet query takes an expert at most 50\% more time compared with a pairwise query, indicating the effectiveness of the proposed $k$-ary query schemes. We generalize the analyses to nonuniform class distributions when possible.

==> ProofTherem3.tex <==
%\begin{proof}
For a dataset with equal class sizes, the probability that the sample $s_1$ settles in the first query $q=1$ is given by
\begin{equation}
\begin{array}{ccl}
P(Q=1) &=& P(s_1 \in \mathcal{L}_1)\\
&=&\sum_{\ell(s_2)=i=0}^{N-2}
P(s_1\in \mathcal{L}_1|(s_1,s_2) \in \mathcal{Q},\\
&&\ell(s_1)=0,\ell(s_2)=i)\\
&\times& P((s_1,s_2)\in \mathcal{Q},\ell(s_1)=0, \ell(s_2)=i)\\
&=&\sum_{\ell(s_2)=i=0}^{N-2}P(s_1\in \mathcal{L}_1|{E}_{i0}=1)\\ 
&\times& P({E}_{i0}=1)\\
&=&\sum_{\ell(s_2)=i=0}^{N-2}P(S_{i,0}) \times P(s_1 \in \mathcal{L}_1|{E}_{i0}=1);
\end{array}    
\end{equation}
Similarly, for $q=2$, we have
\begin{equation}
\begin{array}{ccl}
P(Q=2) &=& P(s_1 \notin \mathcal{L}_1,s_1 \in \mathcal{L}_2)\\
&=&P(s_1 \notin \mathcal{L}_1) \times P(s_1 \in \mathcal{L}_2 | s_1 \notin \mathcal{L}_1)\\
&=& (1-P(s_1 \in \mathcal{L}_1))\\
&\times& \sum_{l(s_2)=i=0}^{N-2} P(S_{i,1}) \times P(s_1 \in \mathcal{L}_2|{E}_{i1}=1);
\end{array}
\end{equation}
And for $q=3$, we have
\begin{equation}
\begin{array}{ccl}
P(Q=3) &=& P(s_1 \notin \mathcal{L}_1,s_1 \notin \mathcal{L}_2,s_1 \in \mathcal{L}_3)\\
&=&P(s_1 \notin \mathcal{L}_1, s_1 \notin \mathcal{L}_2)\\ 
&\times& P(s_1 \in \mathcal{L}_3 | s_1 \notin \mathcal{L}_1, s_1 \notin \mathcal{L}_2)\\
&=&P(s_1 \notin \mathcal{L}_1) \times P(s_1 \notin \mathcal{L}_2|s_1 \notin \mathcal{L}_1)\\
&\times& P(s_1 \in \mathcal{L}_3 | s_1 \notin \mathcal{L}_1, s_1 \notin \mathcal{L}_2)\\
&=& (1-P(s_1 \in \mathcal{L}_1))\\
&\times& (1-P(s_1 \in \mathcal{L}_2|s_1 \notin \mathcal{L}_1))\\ 
&\times& P(s_1 \in \mathcal{L}_3 | s_1 \notin \mathcal{L}_1, s_1 \notin \mathcal{L}_2)\\
&=& (1-P(s_1 \in \mathcal{L}_1))\\
&\times& (1-P(s_1 \in \mathcal{L}_2|s_1 \notin \mathcal{L}_1)) \\
&\times& \sum_{l(s_2)=i=0}^{N-2} P(S_{i,2})
\times P(s_1 \in \mathcal{L}_3|{E}_{i2}=1).
\end{array}
\end{equation}
We can continue the same steps to obtain $P(Q=q)$ as in \eqref{Event1Eq}. The probability $P(s\in \mathcal{L}_{j+1}|{E}_{i,j}=1)$ indicates the probability that a sample $s$ with length $\ell(s)=j$ settles in the next query, when it is paired with a sample of length $i$. The probabilities in \eqref{ProbSuccessEq} is obtained by following the events described in Section~\ref{Algo3Desc} and noting the edge effect when a sample reaches a length of $N-2$ in Algorithm~\ref{Algo3}. Such a sample definitely settles in the next query once it is clear how it compares with one of the remaining two classes. 
%\begin{equation}
%P(s_1\in \mathcal{L}|\mathrm{E}'_{i,j})=
%\begin{cases}
%  \begin{cases}
%p_b (i,j)+p_a(i,j) & i<j \\
%p_c(i,j)+0.5p_d(i,j)+p_a(i,j) & i=j\\
%p_c (i,j)+p_d(i,j)+p_a(i,j) & i>j   
%  \end{cases}
%  & 0 \leq j < N-2\\
%1 & j=N-2
%\end{cases}
%\end{equation}

%\subsubsection{Probability of Success in A Query}
%The probability of successful labeling of $i$ and or $j$ is therefore given by\\
%For $0\leq j \leq i < N-2$
%\begin{itemize}
%    \item 
%	$i$ is successfully labeled: $p_b$ 
%\item
%	$j$ is successfully labeled: $p_c+p_d$
%\item
%	$i$ and $j$ are successfully labeled: $p_a$
%\item
%	None are successfully labeled: $p_e$
%\end{itemize}
%	For $j<i=N-2$
%\begin{itemize}
%    \item 
%	In addition to $i$, $j$ is also labeled: 
%$p_f (N-2,j)=
%p_a (N-2,j)+p_c (N-2,j)+p_d (N-2,j)={3 \over {2(N-j)}}$
%\item
%	Only $i$ is labeled and $j$ is not labeled:\\ 
%$p_g=p_b+p_e={{2N-2j-3} \over {2(N-j)}}$
%\end{itemize}

%	For $j=i=N-2$: 
%	Both are successfully settled

%where $P'_{ij}$ is the probability of the event $\mathrf{E}’_{ij}$ that two samples of length $i$ and $j$ %are paired in one query with a bin; i.e., 
%\begin{equation}
%P'_{ij}=Pr\{E_{ij}=1\}    
%\end{equation}

%\begin{equation}
%E’_{ij}=
%\begin{cases}
%1  & \text{if} \hspace{0.5cm} l(s_1)=i,l(s_2)=j,(s_1,s_2) \in \mathcal{Q}\\
%0  &  \text{otherwise} 
%\end{cases}
%\end{equation}

%And

%\begin{equation}
%P(s_1 \in \mathcal{L},s_2 \in \mathcal{L} | \mathrm{E}'_{ij}=1)= p_a(i,j)    
%\end{equation}

%\begin{equation}
%P(s_1 \in \mathcal{L},s_2 \notin \mathcal{L} | \mathrm{E}'_{ij}=1)=
%\begin{cases}
%P_b(i,j)  &  i>j\\
%P_b(i,j)+P_d(i,j) &  i<j
%\end{cases}
%\end{equation}

%\begin{equation}
%P(s_1 \notin \mathcal{L},s_2 \in \mathcal{L} | \mathrm{E}'_{ij}=1)=
%\begin{cases}
%P_c(i,j)+P_d(i,j)  &  i>j\\
%P_c(i,j) &  i<j
%\end{cases}
%\end{equation}

%Note that $p_b (i,j)= p_c (j,i)$, but the distinction in the last two equations is the result of an assumed advance-queue strategy in which the sample with larger length advances (with the one with smaller length piggy backed on it). 
%\end{proof}
